Multi-Resource Parallel Query Scheduling and Optimization

Scheduling query execution plans is a particularly complex problem in shared-nothing parallel systems, where each site consists of a collection of local time-shared (e.g., CPU(s) or disk(s)) and space-shared (e.g., memory) resources and communicates with remote sites by message-passing. Earlier work on parallel query scheduling employs either (a) one-dimensional models of parallel task scheduling, effectively ignoring the potential benefits of resource sharing, or (b) models of globally accessible resource units, which are appropriate only for shared-memory architectures, since they cannot capture the affinity of system resources to sites. In this paper, we develop a general approach capturing the full complexity of scheduling distributed, multi-dimensional resource units for all forms of parallelism within and across queries and operators. We present a level-based list scheduling heuristic algorithm for independent query tasks (i.e., physical operator pipelines) that is provably near-optimal for given degrees of partitioned parallelism (with a worst-case performance ratio that depends on the number of time-shared and space-shared resources per site and the granularity of the clones). We also propose extensions to handle blocking constraints in logical operator (e.g., hash-join) pipelines and bushy query plans as well as on-line task arrivals (e.g., in a dynamic or multi-query execution environment). Experiments with our scheduling algorithms implemented on top of a detailed simulation model verify their effectiveness compared to existing approaches in a realistic setting. Based on our analytical and experimental results, we revisit the open problem of designing efficient cost models for parallel query optimization and propose a solution that captures all the important parameters of parallel execution.

==> exper.tex <==
%----------------------------------------------------------------------------
\section{Performance Evaluation Using Cost Model Computations}
\label{sec.exper}
%----------------------------------------------------------------------------
In this section, we present the results of several experiments we have conducted
using cost model computations for various query operators in order to examine 
the average-case performance of our scheduling algorithms.
Given our analytical worst-case performance bound on the performance of
our \LevelSched\  algorithm (Theorem~\ref{thm.levelsched}), our main focus in 
this experimental study is to identify how close the response time of the 
generated schedule is to the response time of the optimal execution schedule
{\em on the average}.
This is done using lower bounds on the optimal parallel response time inspired
by Lemma~\ref{lem.newlb}.
 
Our results clearly demonstrate  that the average-case performance of our 
multi-resource scheduling algorithms is much closer to optimal than what would
be predicted by the pessimistic worst-case bound of Theorem~\ref{thm.levelsched}.
Thus, on the average, our scheduling algorithms produce very effective, near-optimal
packings of memory and work requirements over the system sites.
%
%To the best of our knowledge, the issue of complex query scheduling 
%with both \tsr\ and \ssr\ resources has not been addressed in prior
%work on databases or deterministic scheduling theory.
%Given this lack of adversaries, our experiments focus on how close the
%response time of the generated schedule is to a lower bound on the response
%time of the  optimal execution schedule (Lemma~\ref{lem.newlb})
%{\em on the average\/}.
%Note that this also provides an indication of the quality and, perhaps
%most importantly, the consistency of our lower bound as a predictor of
%the expected response time of a query plan.
%
We start by presenting our experimental testbed and methodology.




%--------------------------
\subsection{Experimental Testbed}
\label{sec.testbed}
%--------------------------
We have experimented with the following multi-resource scheduling
algorithms developed in this paper:
\begin{itemize}
\item
\LevelSched\ :
Level-based scheduling of multiple independent query tasks (i.e., operator 
pipelines). %(Figure~\ref{fig.levelsched}).
\item
\TreeSched\ :
Level-based scheduling of query task trees, observing blocking constraints
and execution dependencies  across execution layers (Section~\ref{sec.treesched}).
%in the tree as well as main-memory dependencies across execution 
%levels (Section~\ref{sec.treesched}).
\end{itemize}
For both scheduling scenarios (independent tasks, task trees), we compared
the average performance of our scheduling algorithms with a lower
bound on the response time of the optimal execution schedule for the given
degrees of partitioned parallelism (determined by the granularity parameters
$\lambda$ and $f$).
These lower bounds  for independent query tasks (\LevelBound) and
query task trees (\TreeBound) were estimated using the formulas:
\[
{\small
\mbox{\LevelBound} = \max\{\ms \frac{l(S^{W})}{P} \ms,\ms \frac{l(S^{TV})}{P} \ms,\ms T^{max}(S) \ms\}}
\mbox{\hspace{1.5ex} and \hspace{1.5ex}}
{\small
\mbox{\TreeBound} = \max\{\ms \frac{l(S^{W})}{P} \ms,\ms \frac{l(S^{TV})}{P} \ms,\ms T(\mbox{CP}) \ms\}},
\]
where $S$ is the collection of all operator clones in the query tasks and task
tree (respectively), $T^{max}(S)$ is the maximum  stand-alone execution time
among all clones in $S$, and $T(\mbox{CP})$ is the total response time of the
critical (i.e., most time-consuming) path in the query task tree.


Some additional assumptions were made to obtain a specific experimental model from the
general parallel execution model described in Sections~\ref{sec.partitioned} 
and~\ref{sec.sched}.
These are briefly summarized below:
\begin{description}
\item[EA1.]
{\bf No Data or Execution Skew}: With the exception of startup cost, 
the work and \ssr\ demand vectors of an operator are distributed perfectly 
among all sites participating in its execution.
Startup is  added to the work components of only one of these sites, 
the ``coordinator site'' for the parallel execution.
Furthermore, startup overhead is equally divided between the
coordinator's CPU and its network interface.
\item[EA2.]
{\bf Uniform \tsr\ Resource Overlapping}:
The amount of overlap achieved between processing at different
\tsr\ resources at a site can be characterized by a single
system-wide parameter $\epsilon\in[0,1]$
for all query operators.
This parameter  allows us to express the response time
of a work vector as a convex combination of the maximum
and the sum of the vector components (see Section~\ref{sec.usage}),
i.e.,
\[ T^{seq}(\overline{W}) = \epsilon \max_{1\leq i\leq d}\{ W[i] \} +
                  (1-\epsilon) \sum_{i=1}^{d}W[i].
\]
Small values of $\epsilon$ imply limited overlap,
whereas values closer to 1 imply a larger degree of overlap.
In the extreme cases,
$\epsilon=1$ gives $T(\overline{W}) = \max_{1\leq i\leq d}\{ W[i] \}$
(perfect overlap), and $\epsilon=0$ gives
$T(\overline{W}) = \sum_{i=1}^{d}W[i]$ (zero overlap).
\item[EA3.]
{\bf Simple Hash-Join Plan Nodes}:
The query tasks handed to our algorithms are generated by bushy
hash-join plans, where the memory demand for each join equals the
size of the inner relation times a ``fudge factor'' accounting for the
hash table overhead.
Note that even though it is possible to execute a hash-join with 
less memory~\cite{shapiro:tods86}, such memory limitations complicate the
processing of multi-join pipelines -- since \opprobe\ operators cannot keep 
their entire data sets (i.e., inner hash tables) in memory, it is
no longer possible to execute the \opprobe\ pipeline in one pass.
This means that intermediate disk I/O has to be performed at one or more
pipeline stages, essentially modifying the original plan with the addition
of extra blocking and data dependencies.
Various multi-pass schemes for pipelined hash-join execution under limited 
memory were studied in the work of Schneider~\cite{schneider:phdthesis90}.
As part of our future work, we plan to investigate the effects of such memory
limitations on our scheduling methodology and results.
\end{description}
Finally, we should note that our implementations of \TreeSched\ and \LevelSched\
incorporated an additional optimization to the basic scheme shown in 
Figure~\ref{fig.levelsched}: 
{\em After the placement of a schedulable sublist (Lemma~\ref{lem.ubnosites}) of ready 
pipelines, each remaining ready  pipeline was checked (in non-increasing
order of $T^{max}$) for possible inclusion in the current level before starting
the next execution level.\/}
Although this optimization does not help improve worst-case performance (since
Lemma~\ref{lem.ubnosites} is tight), we found that it really helped the average-case
performance of the heuristics at the cost of a small increase in running time.


We experimented with tree queries of 10, 20, 30, 40, and 50 joins.
For each query size, twenty query graphs (trees) were randomly generated
and for each graph an execution plan was selected in a random
manner from a bushy plan space.
We assumed simple key join operations in which
the size of the result relation
is always equal to the size of the largest of the two
join operands.
For  algorithm \LevelSched, all data dependencies 
in the query task trees were removed  to obtain a collection of
independent tasks from each tree query.
We used two performance metrics in our study:
(1) the {\em expected response time\/} (based on cost model computations)
of the schedules produced by our algorithms; and,
(2) the {\em average performance ratio\/}
defined as the expected response time of the schedules produced by 
our algorithms divided by the corresponding lower bound and averaged
over all queries of the same size.
%
%(2) the {\em expected response time\/} (based on cost of the schedules produced by our
%heuristics over all queries of the same size.
%%In addition to the regular experimental runs in which the plan parameters 
%%were kept fixed  as the system parameters were varied, we also ran some
%%{\em scaleup\/} experiments, where the sizes of the input relations were
%%scaled by the amount of memory available at each site.
Experiments were conducted with the resource overlap parameter $\epsilon$
varying between 10\% and 70\%, the coarse granularity parameter $f$
varying between 0.3 and 0.9, and the \ssr\ granularity parameter $\lambda$
varying between 0.1 and 0.9.
%Since the effects of $f$ and $\epsilon$ on scheduler performance were
%also studied in our prior work~\cite{gi:sigmod96}, the experiments discussed
%in this paper mostly concentrate on the new parameter $\lambda$.
%
The discussion of our experimental results focuses primarily on the effects
of the memory granularity parameter $\lambda$.
We should note, however, that the results presented in the next section
are indicative of the results obtained for all values of $f$ and $\epsilon$.
Further, the response time and lower bound curves (presented for specific query
trees) are qualitatively similar to the curves obtained for other queries of the
same size.
%
%and other system parameters.)


In all experiments, we assumed system nodes consisting of $d=3$ 
\tsr\ resources (one CPU, one disk unit, and one network interface)
and $s=1$ \ssr\ resource (memory).
The work vector components for the CPU and the disk were estimated
using the cost model equations given by Hsiao et al.~\cite{hcy:sigmod94}.
The communication costs were calculated using the linear model briefly 
described in Section~\ref{sec.degree}.
The memory requirement of hash-join operators was estimated as 
$F$ times the size of the inner join relation, where $F$ is the fudge factor
for  hash table overheads~\cite{shapiro:tods86}.
The values of the cost model parameters were obtained from the literature
\cite{hcy:sigmod94,gw:rutgers93,wfa:vldb92} and are summarized in
Table~\ref{tab.params}.

\begin{SingleSpace}

\begin{table}[ht]
\vskip 5pt
\hbox{
{\small
\begin{minipage}{0.5\hsize}
\sloppy
\hfil
\begin{center}
\begin{tabular}{||l|r||} \hline\hline
{\bf Configuration/Catalog Parameters}  &      {\bf Value} \\ \hline\hline
Number of Sites                      &  10 -- 120  \\ \hline
CPU Speed                            &  10 MIPS    \\ \hline
Memory per Site                      &  16 -- 64 MB \\ \hline
Effective Disk Service Time per page &  5 msec   \\ \hline
Startup Cost per site ($\alpha$)     &  25 msec   \\ \hline
Network Transfer Cost per byte ($\beta$) & 0.2 $\mu$sec \\ \hline
Fudge Factor (F)                     & 1.4 \\ \hline
Tuple Size                           & 128 bytes  \\ \hline
Page Size                            & 32 tuples  \\ \hline
Relation Size                        & $10^{4}$ -- $10^{6}$ tuples \\ \hline\hline
\end{tabular}
\end{center}
\hfil
\end{minipage}

\begin{minipage}{0.5\hsize}
\sloppy
\hfil
\begin{tabular}{||l|r||} \hline\hline
{\bf CPU Cost Parameters}                 &    {\bf No. Instr.} \\ \hline\hline
Read Page from Disk                 &         5000        \\ \hline
Write Page to Disk                  &         5000        \\ \hline
Extract Tuple                       &          300        \\ \hline
Hash Tuple                          &          100        \\ \hline
Probe Hash Table                    &          200        \\ \hline\hline
\end{tabular}
\hfil
\end{minipage}
}
}
\caption{Experiment Parameter Settings}
\label{tab.params}
\vskip 5pt
\end{table}

\end{SingleSpace}



%----------------------
\subsection{Experimental Results} 
\label{sec.expresults}
%----------------------
The first set  of experiments studied  the average-case  behavior 
of our level-based \TreeSched\ heuristic for different query, system, and
memory sizes and various settings for the $\lambda$, $f$, and $\epsilon$
parameters.
Figure~\ref{fig.plot1}(a)  depicts the average performance ratio of \TreeSched\
for queries of 40 joins and 32MB of memory at each site, assuming 
a coarse-granularity parameter $f = 0.6$ and a resource overlap of 
$50\%$ (i.e., $\epsilon = 0.5$).
Note that our algorithm is consistently within a small constant
factor (i.e., less than 2) of the lower bound on the optimal schedule length.
Although the distance from the lower bound has certainly increased compared
to our results for only \tsr\ resources (see~\cite{gi:sigmod96}), the results
clearly demonstrate that the worst-case multiplicative factors derived in
our analytical bounds are overly pessimistic as far as average performance is 
concerned.


\begin{SingleSpace}

\depsfig{1.0}{Plots/rat.vs.no_sites-06.05-40J-32MB.eps}
        {1.0}{Plots/rt.vs.no_sites-06.05-40J-32MB.eps}
{Effect of $\lambda$ on (a) the average performance ratio of \TreeSched, and 
(b) the schedule response times obtained by \TreeSched. 
($f = 0.6$, $\epsilon = 0.5$)}
{fig.plot1}

\end{SingleSpace}


Observing Figure~\ref{fig.plot1}(a), it appears that \TreeSched\  performs
better for larger values of the memory granularity parameter $\lambda$.
This is slightly counterintuitive and seems to contradict Section~\ref{sec.pipesched}: 
``finer'' memory requirements should allow our schedulers to obtain better
load balancing and, consequently, better schedules.
However, as shown in Figure~\ref{fig.plot1}(b), although the {\em performance ratio\/} of the
algorithms improves with larger values of $\lambda$, the {\em actual performance\/}
(i.e., the response time) of the schedules deteriorates with larger $\lambda$,
as expected.
The explanation of this phenomenon lies in Figure~\ref{fig.plot2} which shows how the three
components of the \TreeBound\ lower bound vary with the number of sites for our example
%%set of 
40-join query tree and  16MB of memory per site.
(We chose a smaller value for memory because it better illustrates the effect of 
the volume term for our system setting.) 

\begin{SingleSpace}

\depsfig{1.0}{Plots/lbound.vs.no_sites-06.05-40J-16MB-0.2l.eps}
        {1.0}{Plots/lbound.vs.no_sites-06.05-40J-16MB-0.8l.eps}
{\TreeBound\ components for (a)  $\lambda = 0.2$, and
(b) $\lambda = 0.8$. ($f = 0.6$, $\epsilon = 0.5$)}
{fig.plot2}

\end{SingleSpace}

Note that for small values of the number of sites $P$ the dominant factor in \TreeBound\
is the average volume term ($\frac{l(S^{TV})}{P}$).
For larger values of $P$ (and, consequently, increased system memory), \TreeBound\ is 
determined by the average work term ($\frac{l(S^{W})}{P}$).
Eventually, as $P$ continues to grow, the critical path term ($T(\mbox{CP})$)
starts dominating the other two terms in the bound.
Also, note that as the critical path becomes the dominant factor
in the query plan execution, our level-based methods  become more accurate
in approximating the lower bound.
Intuitively, this is because the ``height'' of each execution level as determined by the
plan's critical path will be sufficient to pack the work in that level and, thus, the
resource loss due to ``shelving'' is not important.
(This also explains why the average performance ratios for various values of $\lambda$ 
all converge to a value close to unity as the number of sites is increased.)
For the parameter settings in our experiments, larger values for the memory 
granularity $\lambda$ typically  imply  lower degrees of  parallelism 
for the operators in the plan, which means that the critical path will start dominating
the other two factors in \TreeBound\ much sooner.
Furthermore, the aforementioned effect  on the performance ratio becomes more 
pronounced since the critical path term will be significantly larger for larger
$\lambda$ (Figure~\ref{fig.plot3}).
Consequently, larger values for $\lambda$ imply better performance ratios 
(Figure~\ref{fig.plot1}(a)), even though the actual schedule response times
are worse (Figure~\ref{fig.plot1}(b)).

For our second set of experiments, we removed all the blocking and data 
dependencies from the query task trees and scheduled the resulting collection
of independent query tasks using \LevelSched.
Again, we focused on the effect of $\lambda$ on the performance of our
scheduling heuristic for different query and system sizes and different 
amounts of memory per site.
The average performance ratio and expected response time plots for schedules 
obtained for various values of $\lambda$ with $f=0.6$ and $\epsilon=0.5$ are
shown in Figures~\ref{fig.plot3}(a) and \ref{fig.plot3}(b), respectively.
With respect to our previous discussion, the main observation here is that 
when all dependencies are removed, smaller values of $\lambda$ (i.e., ``finer''
clones) result in both better response times {\em and\/}  better performance ratios.
The reason is that, in the absence of scheduling constraints, finer clones allow 
\LevelSched\ to produce better packings and minimize resource wastage within 
each level.
Also, note that both curves are significantly better (i.e., lower) than those
of \TreeSched, since the lack of dependencies allows \LevelSched\ to obtain
better execution schedules.


\begin{SingleSpace}

\depsfig{1.0}{Plots/rat.vs.no_sites-06.05-40J-32MB-NODEP.eps}
        {1.0}{Plots/rt.vs.no_sites-06.05-40J-32MB-NODEP.eps}
{Effect of $\lambda$ on (a) the average performance ratio of \LevelSched, and
(b) the average schedule response times obtained by \LevelSched. 
($f = 0.6$, $\epsilon = 0.5$)}
{fig.plot3}

\end{SingleSpace}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\eat{
Finally, we ran some scaleup experiments with \TreeSched, in which the
size of the input (base) relations of the query plan were scaled according
to the amount of memory available at each site assuming a base configuration
with 16MB per site.
Thus, for example, when each site had 32MB of memory the base relation sizes in
all plans were multiplied by two.
Figure~\ref{fig.plot4} shows the average response times obtained by \TreeSched\
on 50-join queries for 32MB and 48MB of memory per site.

\begin{SingleSpace}

\depsfig{1.0}{Plots/rt.vs.no_sites-06.05-50J-32MB-SCALEUP.eps}
        {1.0}{Plots/rt.vs.no_sites-06.05-50J-48MB-SCALEUP.eps}
{Average response times obtained by \TreeSched\ for scaleup
experiments with  (a) 32MB of memory per site, and
(b) 48MB of memory per site.
($f = 0.6$, $\epsilon = 0.5$)}
{fig.plot4}

\end{SingleSpace}
}

